The top quark electro-weak couplings after LHC Run 2

Recent measurements at the Large Hadron Collider allow for a robust and precise characterisation of the electro-weak interactions of the top quark. We present the results of a global analysis at next-to-leading order precision including LHC, LEP/SLD and Tevatron data in the framework of the Standard Model Effective Field Theory. We include a careful analysis of the impact of correlations among measurements, as well as of the uncertainties in the Effective Field Theory setup itself. We find remarkably robust global fit results, with central values in good agreement with the Standard Model prediction, and 95% probability bounds on Wilson coefficients that range from $\pm$ 0.35 to $\pm$ 8 TeV$^{-2}$. This result represents a considerable improvement over previous studies, thanks to the addition of differential cross-section measurements in associated production processes of top quarks and neutral gauge bosons.

==> tab_param/tab_param.tex <==
\newpage
% \newgeometry{top=1.5cm, bottom=2cm}
\begin{sidewaystable}[!htb]    
    \renewcommand\arraystretch{1.5}
    \begin{adjustwidth}{-2cm}{-2cm}
        \footnotesize
        \centering
        \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
            \hline
            13~TeV & Param. [fb] & $\mathcal{O}_{tZ}$ & $\mathcal{O}_{tW}$ & $\mathcal{O}_{\varphi Q}^{(3)}$ & $\mathcal{O}_{\varphi Q}^{(-)}$ & $\mathcal{O}_{\varphi t}$ & $\mathcal{O}_{tG}$ & $\mathcal{O}_{t\varphi}$ & $\mathcal{O}_{bW}$ & $\mathcal{O}_{\varphi tb}$ \\ \hline
            %TTZ
            \multirow{3}{*}{$t\bar{t}Z$}  & $\sigma_{SM,NLO}$ & \multicolumn{9}{c}{$740.8^{+9.7\%}_{-11\%}$} \\ \cline{3-11}
            & $\frac{\sigma_{i,NLO}^{(1)}}{\sigma_{SM,NLO}}\times\%$ & $-0.4^{+38\%}_{-15\%}$ & $-$ & $-$ & $-10.3^{+1.1\%}_{-0.1\%}$ & $6.6^{+1.3\%}_{-0.2\%}$ & $38.9^{+0.9\%}_{-0.9\%}$ & $-$ & $-$ & $-$ \\
            & $\frac{\sigma_{i,NLO}^{(2)}}{\sigma_{SM,NLO}}\times\%$ & $8.4^{+0.8\%}_{-1.4\%}$ & $-$ & $-$ & $0.5^{+0.2\%}_{-2.2\%}$ & $0.4^{+1.6\%}_{-1.2\%}$ & $39.4^{+10\%}_{-6.5\%}$ & $-$ & $-$ & $-$ \\ \hline
            
            %TZQ
            \multirow{3}{*}{$tZq$}  & $\sigma_{SM,NLO}$ & \multicolumn{9}{c}{$807.7^{+2.2\%}_{-1.7\%}$} \\ \cline{3-11}
            & $\frac{\sigma_{i,NLO}^{(1)}}{\sigma_{SM,NLO}}\times\%$ & $-0.7^{+3.1\%}_{-1.5\%}$ & $2.1^{+0.5\%}_{-0.2\%}$ & $21.8^{+0.3\%}_{-0.1\%}$ & $2.3^{+1.0\%}_{-0.8\%}$ & $0.6^{+1.9\%}_{-0.1\%}$ & $-0.5^{+14\%}_{-17\%}$ & $-$ & $-$ & $-$ \\
            & $\frac{\sigma_{i,NLO}^{(2)}}{\sigma_{SM,NLO}}\times\%$ & $1.9^{+1.2\%}_{-0.2\%}$ & $10.1^{+1.6\%}_{-0.5\%}$ & $3.1^{+1.0\%}_{-1.0\%}$ & $0.2^{+7.0\%}_{-2.3\%}$ & $0.1^{+6.3\%}_{-7.6\%}$ & $0.7^{+27\%}_{-25\%}$ & $-$ & $6.0^{+2.3\%}_{-0.4\%}$ & $0.4^{+1.4\%}_{-0.5\%}$ \\ \hline     
            
            %TTY
            \multirow{3}{*}{$t\bar{t}\gamma$}  & $\sigma_{SM,NLO}$ & \multicolumn{9}{c}{$1986.0^{+10.6\%}_{-11.5\%}$} \\ \cline{3-11}
            & $\frac{\sigma_{i,NLO}^{(1)}}{\sigma_{SM,NLO}}\times\%$ & $-4.2^{+8.3\%}_{-6.3\%}$ & $5.5^{+6.6\%}_{-3.0\%}$ & $-$ & $-$ & $-$ & $29.1^{+1.3\%}_{-0.4\%}$ & $-$ & $-$ & $-$ \\
            & $\frac{\sigma_{i,NLO}^{(2)}}{\sigma_{SM,NLO}}\times\%$ & $14.6^{+0.2\%}_{-0.5\%}$ & $19.1^{+0.6\%}_{-0.3\%}$ & $-$ & $-$ & $-$ & $7.7^{+14\%}_{-3.0\%}$ & $-$ & $-$ & $-$ \\ \hline
            
            %TYQ
            \multirow{3}{*}{$t\gamma q$}  & $\sigma_{SM,NLO}$ & \multicolumn{9}{c}{$869.5^{+2.0\%}_{-1.9\%}$} \\ \cline{3-11}
            & $\frac{\sigma_{i,NLO}^{(1)}}{\sigma_{SM,NLO}}\times\%$ & $-0.6^{+8.5\%}_{-13\%}$ & $2.9^{+2.9\%}_{-2.2\%}$ & $12.1^{+0.1\%}_{-0.1\%}$ & $-$ & $0.1^{+13\%}_{-17\%}$ & $0.5^{+20\%}_{-17\%}$ & $-$ & $-$ & $-$ \\
            & $\frac{\sigma_{i,NLO}^{(2)}}{\sigma_{SM,NLO}}\times\%$ & $5.3^{+0.2\%}_{-0.1\%}$ & $6.6^{+1.2\%}_{-0.2\%}$ & $0.4^{+0.3\%}_{-2.4\%}$ & $-$ & $<10^{-3}$ & $-0.7^{+76\%}_{-14\%}$ & $-$ & $1.5^{+1.3\%}_{-0.1\%}$ & $0.1^{+1.1\%}_{-0.7\%}$ \\ \hline
        
        \end{tabular}
    \end{adjustwidth}
    \caption{Parameterisations for some of the considered processes in the global fit at 13~TeV. Cells with $-$ indicate that they contribute very little and are not included in the fit.}
    \label{tab:fit_process2_13}    
\end{sidewaystable}

\newpage
% \newgeometry{top=1.5cm, bottom=2cm}
\begin{sidewaystable}[!htb]    
    \renewcommand\arraystretch{1.5}
    \begin{adjustwidth}{-2cm}{-2cm}
        \footnotesize
        \centering
        \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
            \hline
            13~TeV & Param. [fb] & $\mathcal{O}_{tZ}$ & $\mathcal{O}_{tW}$ & $\mathcal{O}_{\varphi Q}^{(3)}$ & $\mathcal{O}_{\varphi Q}^{(-)}$ & $\mathcal{O}_{\varphi t}$ & $\mathcal{O}_{tG}$ & $\mathcal{O}_{t\varphi}$ & $\mathcal{O}_{bW}$ & $\mathcal{O}_{\varphi tb}$ \\ \hline
                        
            %TTW
            \multirow{3}{*}{$t\bar{t}W$}  & $\sigma_{SM,NLO}$ & \multicolumn{9}{c}{$543^{+11\%}_{-10\%}$} \\ \cline{3-11}
            & $\frac{\sigma_{i,NLO}^{(1)}}{\sigma_{SM,NLO}}\times \%$ & $-$ & $-$ & $-$ & $-$ & $-$ & $29.1^{+0.7\%}_{-0.2\%}$ & $-$ & $-$ & $-$ \\
            & $\frac{\sigma_{i,NLO}^{(2)}}{\sigma_{SM,NLO}}\times \%$ & $-$ & $-$ & $-$ & $-$ & $-$ & $4.3^{+33\%}_{-19\%}$ & $-$ & $-$ & $-$ \\ \hline
            
            %TTWQ EW
            \multirow{3}{*}{$t\bar{t}W$ EW}  & $\sigma_{SM,NLO}$ & \multicolumn{9}{c}{$47.5^{+19.5\%}_{-15.1\%}$} \\ \cline{3-11}
            & $\frac{\sigma_{i,NLO}^{(1)}}{\sigma_{SM,NLO}}\times\%$ & $-1.0^{+7.9\%}_{-5.4\%}$ & $25.2^{+8.1\%}_{-6.0\%}$ & $7.6^{+0.1\%}_{-0.3\%}$ & $-7.6^{+0.9\%}_{-0.9\%}$ & $3.7^{+3.1\%}_{-2.6\%}$ & $10.3^{+0.9\%}_{-1.0\%}$ & $-$ & $-$ & $-$ \\
            & $\frac{\sigma_{i,NLO}^{(2)}}{\sigma_{SM,NLO}}\times\%$ & $2.3^{+10\%}_{-7.1\%}$ & $57.5^{+4.3\%}_{-3.1\%}$ & $6.2^{+3.5\%}_{-2.5\%}$ & $1.6^{+2.2\%}_{-2.2\%}$ & $1.6^{+3.2\%}_{-2.4\%}$ & $2.4^{+7.9\%}_{-8.8\%}$ & $-$ & $-$ & $-$ \\ \hline

            %TTH
            \multirow{3}{*}{$t\bar{t}H$}  & $\sigma_{SM,NLO}$ & \multicolumn{9}{c}{$459^{+6.3\%}_{-9.3\%}$} \\ \cline{3-11}
            & $\frac{\sigma_{i,NLO}^{(1)}}{\sigma_{SM,NLO}}\times \%$ & $-$ & $-$ & $-$ & $-$ & $-$ & $99.8^{+0.6\%}_{-0.2\%}$ & $-12.9^{+1.8\%}_{-1.0\%}$ & $-$ & $-$ \\
            & $\frac{\sigma_{i,NLO}^{(2)}}{\sigma_{SM,NLO}}\times \%$ & $-$ & $-$ & $-$ & $-$ & $-$ & $130^{+1.2\%}_{-1.7\%}$ & $0.4^{+4.3\%}_{-1.8\%}$ & $-$ & $-$ \\ \hline
            
            %THQ
            \multirow{3}{*}{$tHq$}  & $\sigma_{SM,(N)LO}$ & \multicolumn{7}{c|}{$71.2^{+1.9\%}_{-1.6\%}$ (NLO)} & \multicolumn{2}{c}{$66.6^{+2.5\%}_{-4.3\%}$ (LO)} \\ \cline{3-11}
            & $\frac{\sigma_{i,(N)LO}^{(1)}}{\sigma_{SM,(N)LO}}\times\%$ & $-$ & $29.6^{+1.6\%}_{-1.5\%}$ & $-11.6^{+3.3\%}_{-2.3\%}$ & $-$ & $-$ & $-0.2^{+32\%}_{-38\%}$ & $-0.7^{+16\%}_{-18\%}$ & $0.1^{+0.1\%}_{-0.1\%}$ & $0.01^{+43\%}_{-45\%}$ \\
            & $\frac{\sigma_{i,(N)LO}^{(2)}}{\sigma_{SM,(N)LO}}\times\%$ & $-$ & $78.8^{+0.6\%}_{-0.1\%}$ & $18.8^{+0.6\%}_{-0.2\%}$ & $-$ & $-$ & $-1.9^{+23\%}_{-22\%}$ & $1.1^{+0.6\%}_{-0.4\%}$ & $2.9^{+0.1\%}_{-0.9\%}$ & $0.1^{+1.7\%}_{-1.9\%}$ \\ \hline

        \end{tabular}
    \end{adjustwidth}
    \caption{Continuation of Table~\ref{tab:fit_process2_13}. Parameterisations for some of the considered processes in the global fit at 13~TeV. Cells with $-$ indicate that they contribute very little and are not included in the fit.}% $t\bar{t}W$ EW is shown here for easier comparison with $t\bar{t}W$ QCD production.
    \label{tab:fit_process1_13}    
\end{sidewaystable}


% \newpage
% \begin{sidewaystable}[!htb]    
%     \renewcommand\arraystretch{1.5}
%     \begin{adjustwidth}{-2cm}{-2cm}
%         \footnotesize
%         \centering
%         \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
%             \hline
%             13~TeV & Param. [fb] & $\mathcal{O}_{tZ}$ & $\mathcal{O}_{tW}$ & $\mathcal{O}_{\varphi Q}^{(3)}$ & $\mathcal{O}_{\varphi Q}^{(-)}$ & $\mathcal{O}_{\varphi t}$ & $\mathcal{O}_{tG}$ & $\mathcal{O}_{t\varphi}$ & $\mathcal{O}_{bW}$ & $\mathcal{O}_{\varphi tb}$ \\ \hline
            
%             %TWZ
%             \multirow{3}{*}{$tWZ$}  & $\sigma_{SM,LO}$ & \multicolumn{9}{c}{$107.1^{+10.7\%}_{-10.6\%}$} \\ \cline{3-11}
%             & $\sigma_{i,LO}^{(1)}$ & $-0.37^{+10.3\%}_{-10.1\%}$ & $-11.68^{+10.2\%}_{-9.1\%}$ & $20.69^{+10.9\%}_{-10.9\%}$ & $2.28^{+9.6\%}_{-10.6\%}$ & $1.83^{+11.3\%}_{-11.1\%}$ & $-0.90^{+19.2\%}_{-30.4\%}$ & $0.01^{+10.8\%}_{-10.6\%}$ & $-0.02^{+10.3\%}_{-9.5\%}$ & $0.01^{+10.3\%}_{-9.4\%}$ \\
%             & $\sigma_{i,LO}^{(2)}$ & $4.86^{+7.7\%}_{-7.0\%}$ & $22.84^{+9.8\%}_{-8.6\%}$ & $4.85^{+9.1\%}_{-8.8\%}$ & $0.39^{+14.0\%}_{-10.6\%}$ & $0.19^{+13.1\%}_{-9.4\%}$ & $-1.80^{+3.8\%}_{-30.4\%}$ & $-0.001^{+58.3\%}_{-10.6\%}$ & $17.54^{+9.5\%}_{-7.8\%}$ & $0.78^{+9.6\%}_{-7.7\%}$ \\
%             & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times \%$ & $-0.35^{+21.0\%}_{-20.7\%}$ & $-10.90^{+20.9\%}_{-19.8\%}$ & $19.32^{+21.7\%}_{-21.6\%}$ & $2.12^{+20.4\%}_{-21.3\%}$ & $1.70^{+22.1\%}_{-21.8\%}$ & $-0.84^{+30.0\%}_{-41.0\%}$ & $0.001^{+21.6\%}_{-21.3\%}$ & $-0.02^{+21.0\%}_{-20.2\%}$ & $0.01^{+21.0\%}_{-20.1\%}$ \\
%             & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times \%$ & $4.54^{+18.5\%}_{-17.7\%}$ & $21.32^{+20.5\%}_{-19.2\%}$ & $4.53^{+19.9\%}_{-19.5\%}$ & $0.36^{+24.7\%}_{-21.3\%}$ & $0.18^{+23.8\%}_{-20.1\%}$ & $-1.68^{+14.5\%}_{-41.0\%}$ & $-0.001^{+69.0\%}_{-21.3\%}$ & $16.41^{+20.2\%}_{-18.4\%}$ & $0.73^{+20.3\%}_{-18.4\%}$ \\ \hline
            
%             %TWY
%             \multirow{3}{*}{$tW\gamma$}  & $\sigma_{SM,LO}$ & \multicolumn{9}{c}{$203.1^{+12.9\%}_{-12.6\%}$} \\ \cline{3-11}
%             & $\sigma_{i,LO}^{(1)}$ & $-4.98^{+11.6\%}_{-12.7\%}$ & $-11.52^{+12.3\%}_{-12.0\%}$ & $24.95^{+12.9\%}_{-12.6\%}$ & $0.18^{+12.9\%}_{-12.6\%}$ & $-0.11^{+12.9\%}_{-12.6\%}$ & $13.80^{+12.7\%}_{-12.4\%}$ & $0.02^{+12.9\%}_{-12.6\%}$ & $0.02^{+12.4\%}_{-12.1\%}$ & $-0.01^{+12.9\%}_{-12.6\%}$ \\
%             & $\sigma_{i,LO}^{(2)}$ & $20.01^{+8.2\%}_{-8.1\%}$ & $23.51^{+9.6\%}_{-9.3\%}$ & $0.87^{+12.9\%}_{-12.6\%}$ & $0.24^{+12.9\%}_{-12.6\%}$ & $0.03^{+12.9\%}_{-12.6\%}$ & $33.20^{+8.4\%}_{-8.1\%}$ & $0.001^{+12.9\%}_{-12.6\%}$ & $9.16^{+9.3\%}_{-9.0\%}$ & $0.19^{+12.9\%}_{-12.6\%}$ \\
%             & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times \%$ & $-2.45^{+24.5\%}_{-25.3\%}$ & $-5.67^{+25.2\%}_{-24.6\%}$ & $12.28^{+25.8\%}_{-25.2\%}$ & $0.09^{+25.8\%}_{-25.2\%}$ & $-0.06^{+25.8\%}_{-25.2\%}$ & $6.79^{+25.6\%}_{-25.0\%}$ & $0.01^{+25.8\%}_{-25.2\%}$ & $0.01^{+25.3\%}_{-24.7\%}$ & $-0.001^{+25.8\%}_{-25.2\%}$ \\
%             & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times \%$ & $9.85^{+21.1\%}_{-20.7\%}$ & $11.58^{+22.5\%}_{-21.9\%}$ & $0.43^{+25.8\%}_{-25.2\%}$ & $0.12^{+25.8\%}_{-25.2\%}$ & $0.01^{+25.8\%}_{-25.2\%}$ & $16.35^{+21.3\%}_{-20.7\%}$ & $0.001^{+25.8\%}_{-25.2\%}$ & $4.50^{+22.2\%}_{-21.6\%}$ & $0.09^{+25.8\%}_{-25.2\%}$ \\ \hline

%             %TWH
%             \multirow{3}{*}{$tWH$}  & $\sigma_{SM,LO}$ & \multicolumn{9}{c}{$16.0^{+10.3\%}_{-10.1\%}$} \\ \cline{3-11}
%             & $\sigma_{i,LO}^{(1)}$ & $-0.01^{+10.3\%}_{-10.1\%}$ & $-2.78^{+8.3\%}_{-8.6\%}$ & $5.84^{+9.1\%}_{-9.9\%}$ & $-0.02^{+10.3\%}_{-10.1\%}$ & $-0.001^{+10.3\%}_{-10.1\%}$ & $4.15^{+10.3\%}_{-10.5\%}$ & $-1.68^{+10.1\%}_{-9.4\%}$ & $0.001^{+10.1\%}_{-9.9\%}$ & $-0.001^{+10.3\%}_{-10.2\%}$ \\
%             & $\sigma_{i,LO}^{(2)}$ & $0.001^{+10.3\%}_{-10.1\%}$ & $7.61^{+10.9\%}_{-10.3\%}$ & $2.83^{+11.0\%}_{-11.1\%}$ & $0.001^{+10.3\%}_{-10.1\%}$ & $-0.001^{+10.3\%}_{-10.1\%}$ & $13.10^{+9.8\%}_{-6.9\%}$ & $0.16^{+10.1\%}_{-9.3\%}$ & $0.51^{+8.6\%}_{-8.4\%}$ & $0.01^{+10.3\%}_{-11.3\%}$ \\
%             & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times \%$ & $-0.08^{+20.6\%}_{-20.2\%}$ & $-17.35^{+18.6\%}_{-18.7\%}$ & $36.44^{+19.4\%}_{-20.0\%}$ & $-0.12^{+20.6\%}_{-20.2\%}$ & $-0.02^{+20.6\%}_{-20.2\%}$ & $25.87^{+20.6\%}_{-20.6\%}$ & $-10.50^{+20.4\%}_{-19.5\%}$ & $0.02^{+20.4\%}_{-20.1\%}$ & $-0.02^{+20.6\%}_{-20.3\%}$ \\
%             & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times \%$ & $0.02^{+20.6\%}_{-20.2\%}$ & $47.44^{+21.2\%}_{-20.4\%}$ & $17.63^{+21.3\%}_{-21.2\%}$ & $0.02^{+20.6\%}_{-20.2\%}$ & $-0.001^{+20.6\%}_{-20.2\%}$ & $81.67^{+20.1\%}_{-17.0\%}$ & $1.01^{+20.4\%}_{-19.4\%}$ & $3.17^{+18.9\%}_{-18.5\%}$ & $0.09^{+20.6\%}_{-21.4\%}$ \\ \hline

%         \end{tabular}
%     \end{adjustwidth}
%     \caption{Wilson coefficients for future processes at 13~TeV.}
%     \label{tab:future_process_13}
% \end{sidewaystable}

\newpage
\begin{sidewaystable}[!htb]    
    \renewcommand\arraystretch{1.5}
    \begin{adjustwidth}{-2cm}{-2cm}
        \footnotesize
        \centering
        \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
            \hline
            8~TeV & Param. [pb] & $\mathcal{O}_{tZ}$ & $\mathcal{O}_{tW}$ & $\mathcal{O}_{\varphi Q}^{(3)}$ & $\mathcal{O}_{\varphi Q}^{(-)}$ & $\mathcal{O}_{\varphi t}$ & $\mathcal{O}_{tG}$ & $\mathcal{O}_{t\varphi}$ & $\mathcal{O}_{bW}$ & $\mathcal{O}_{\varphi tb}$ \\ \hline
            
            %tj tchan
            \multirow{3}{*}{$tq$ (t-ch)}  & $\sigma_{SM,NLO}$ & \multicolumn{9}{c}{$82.6^{+2.6\%}_{-2.2\%}$} \\ \cline{3-11}
            & $\frac{\sigma_{i,NLO}^{(1)}}{\sigma_{SM,NLO}}\times\%$ & $-$ & $3.1^{+0.5\%}_{-0.2\%}$ & $11.7^{+0.4\%}_{-0.5\%}$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
            & $\frac{\sigma_{i,NLO}^{(2)}}{\sigma_{SM,NLO}}\times\%$ & $-$ & $1.5^{+2.0\%}_{-1.2\%}$ & $0.2^{+2.3\%}_{-6.8\%}$ & $-$ & $-$ & $-$ & $-$ & $0.5^{+2.4\%}_{-1.2\%}$ & $0.1^{+1.8\%}_{-1.5\%}$ \\ \hline         
            
            %TW
            \multirow{3}{*}{$tW$}  & $\sigma_{SM,NLO}$ & \multicolumn{9}{c}{$22.4^{+6.8\%}_{-6.7\%}$} \\ \cline{3-11}
            & $\frac{\sigma_{i,NLO}^{(1)}}{\sigma_{SM,LO}}\times\%$ & $-$ & $-8.8^{+0.3\%}_{-0.4\%}$ & $12.1^{+0.3\%}_{-0.2\%}$ & $-$ & $-$ & $7.5^{+1.7\%}_{-1.6\%}$ & $-$ & $-$ & $-$ \\
            & $\frac{\sigma_{i,NLO}^{(2)}}{\sigma_{SM,LO}}\times\%$ & $-$ & $2.2^{+0.7\%}_{-0.5\%}$ & $0.4^{+7.0\%}_{-1.6\%}$ & $-$ & $-$ & $-$ & $-$ & $1.0^{+1.3\%}_{-2.7\%}$ & $0.1^{+0.7\%}_{-0.4\%}$ \\ \hline           
            
            %tb schan
            \multirow{3}{*}{$tb$ (s-ch)}  & $\sigma_{SM,NLO}$ & \multicolumn{9}{c}{$4843.0^{+3.6\%}_{-3.3\%}$} \\ \cline{3-11}
            & $\frac{\sigma_{i,NLO}^{(1)}}{\sigma_{SM,NLO}}\times\%$ & $-$ & $46.9^{+0.1\%}_{-0.1\%}$ & $12.3^{+0.1\%}_{-0.1\%}$ & $-$ & $-$ & $-0.1^{+23\%}_{-18\%}$ & $-$ & $-$ & $-$ \\
            & $\frac{\sigma_{i,NLO}^{(2)}}{\sigma_{SM,NLO}}\times\%$ & $-$ & $8.8^{+0.2\%}_{-0.5\%}$ & $0.6^{+4.0\%}_{-3.2\%}$ & $-$ & $-$ & $1.8^{+9.8\%}_{-2.9\%}$ & $-$ & $3.7^{+0.3\%}_{-0.1\%}$ & $0.1^{+0.5\%}_{-0.1\%}$ \\ \hline \hline  
            
            %tj schan TEVATRON
            \multirow{3}{*}{$tb$ (s-ch) @ 1.96~TeV}  & $\sigma_{SM,LO}$ & \multicolumn{9}{c}{$0.7^{+9.3\%}_{-8.1\%}$} \\ \cline{3-11}
            & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times\%$ & $-$ & $46.1^{+0.1\%}_{-0.1\%}$ & $12.1^{+0.1\%}_{-0.1\%}$ & $-$ & $-$ & $<10^{-3}$ & $-$ & $-$ & $-$ \\
            & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times\%$ & $-$ & $7.3^{+0.9\%}_{-0.5\%}$ & $0.4^{+1.5\%}_{-2.2\%}$ & $-$ & $-$ & $1.2^{+4.2\%}_{-6.3\%}$ & $-$ & $3.1^{+0.5\%}_{-0.3\%}$ & $0.1^{+0.1\%}_{-0.1\%}$ \\ \hline 
            
        
            % %FL
            % \multirow{3}{*}{W-hel. FL OLD}  & $F_{SM,LO}$ & \multicolumn{9}{c}{0.3} \\ \cline{3-11}
            % & $F_{i,LO}^{(1)}\times 10^{3}$ & $-$ & 59.8 & $-$0.26 & $-$ & $-$ & $-$ & $-$ & $-$0.54 & 0.0 \\
            % & $F_{i,LO}^{(2)}\times 10^{3}$ & $-$ & $-$3.29 & $-$0.25 & $-$ & $-$ & $-$ & $-$ & $-$6.11 & $-$2.08 \\ \hline
            
            % %F0
            % \multirow{3}{*}{W-hel. F0 OLD}  & $F_{SM,LO}$ & \multicolumn{9}{c}{0.7} \\ \cline{3-11}
            % & $F_{i,LO}^{(1)}\times 10^{3}$ & $-$ & $-$61.3 & 0.26 & $-$ & $-$ & $-$ & $-$ & 0.49 & 0.0 \\
            % & $F_{i,LO}^{(2)}\times 10^{3}$ & $-$ & 3.29 & 0.25 & $-$ & $-$ & $-$ & $-$ & $-$6.11 & 1.04 \\ \hline

            %FL
            % \multirow{3}{*}{W-hel. FL}  & $F_{SM,LO}$ & \multicolumn{9}{c}{0.296} \\ \cline{3-11}
            % & $F_{i,LO}^{(1)}\times 10^{3}$ & $-$ & 56.9 & $-$0.08 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
            % & $F_{i,LO}^{(2)}\times 10^{3}$ & $-$ & $-$2.3 & $-$0.02 & $-$ & $-$ & $-$ & $-$ & $-$1.1 & $-$0.1 \\ \hline
            
            %F0
            % \multirow{3}{*}{W-hel. F0}  & $F_{SM,LO}$ & \multicolumn{9}{c}{0.704} \\ \cline{3-11}
            % & $F_{i,LO}^{(1)}\times 10^{3}$ & $-$ & $-$56.9 & 0.08 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
            % & $F_{i,LO}^{(2)}\times 10^{3}$ & $-$ & 2.3 & 0.02 & $-$ & $-$ & $-$ & $-$ & $-$2.2 & 0.001 \\ \hline
        \end{tabular}
    \end{adjustwidth}
    \caption{Parameterisations for each of the considered processes in the global fit at 8~TeV. Cells with $-$ indicate that they contribute very little and are not included in the fit.}
    \label{tab:fit_process_8}
\end{sidewaystable}
\newpage

% \begin{table}[!htpb]
%     \centering
%     \scriptsize
%     \renewcommand\arraystretch{1.5}
%     \begin{tabular}{c|c|c|c}
%         \hline
%         Process & Param. [pb] & $\mathcal{O}_{ut}^8$ & $\mathcal{O}_{dt}^8$ \\ \hline
        
%         %TT TEVATRON
%         \multirow{3}{*}{$t\bar{t}$ @ 1.96~TeV}  & $\sigma_{SM,LO}$ & \multicolumn{2}{c}{$4.95^{+38\%}_{-26\%}$} \\ \cline{3-4}
%         & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times\%$ & $6.2^{+1.2\%}_{-0.5\%}$ & $1.0^{+7.4\%}_{-2.5\%}$ \\
%         & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times\%$ & $0.5^{+1.7\%}_{-3.0\%}$ & $0.1^{+9.7\%}_{-11\%}$ \\ \hline
                
%         % TT 8TEV
%         \multirow{3}{*}{$t\bar{t}$ @ 8~TeV}  & $\sigma_{SM,LO}$ & \multicolumn{2}{c}{$138^{+33\%}_{-23\%}$} \\ \cline{3-4}
%         & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times\%$ & $1.3^{+6.3\%}_{-2.1\%}$ & $0.8^{+9.8\%}_{-3.3\%}$ \\
%         & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times\%$ & $0.2^{+6.1\%}_{-6.7\%}$ & $0.1^{+9.9\%}_{-11\%}$ \\ \hline
                
%         % TT 13TEV
%         \multirow{3}{*}{$t\bar{t}$ @ 13~TeV}  & $\sigma_{SM,LO}$ & \multicolumn{2}{c}{$453^{+28\%}_{-20\%}$} \\ \cline{3-4}
%         & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times \%$ & $0.9^{+8.7\%}_{-3.0\%}$ & $0.6^{+13\%}_{-4.3\%}$ \\
%         & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times \%$ & $0.2^{+5.8\%}_{-6.2\%}$ & $0.1^{+13\%}_{-13\%}$ \\ \hline
        
%         %TTH
%         \multirow{3}{*}{$t\bar{t}H$ @ 13~TeV}  & $\sigma_{SM,LO}$ & \multicolumn{2}{c}{$0.36^{+29\%}_{-21\%}$} \\ \cline{3-4}
%         & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times \%$ & $5.7^{+6.1\%}_{-3.4\%}$ & $3.5^{+9.4\%}_{-5.2\%}$ \\
%         & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times \%$ & $2.5^{+3.8\%}_{-1.7\%}$ & $1.3^{+6.4\%}_{-2.8\%}$ \\ \hline    
       
%         %TTY
%         \multirow{3}{*}{$t\bar{t}\gamma$ @ 13~TeV}  & $\sigma_{SM,LO}$ & \multicolumn{2}{c}{$1.32^{+29\%}_{-21\%}$} \\ \cline{3-4}
%         & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times \%$ & $2.7^{+6.2\%}_{-4.1\%}$ & $1.6^{+9.8\%}_{-6.5\%}$ \\
%         & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times \%$ & $1.1^{+5.1\%}_{-2.6\%}$ & $0.8^{+7.7\%}_{-4.0\%}$ \\ \hline    
        
%         %TTZ
%         \multirow{3}{*}{$t\bar{t}Z$ @ 13~TeV}  & $\sigma_{SM,LO}$ & \multicolumn{2}{c}{$0.51^{+30\%}_{-21\%}$} \\ \cline{3-4}
%         & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times \%$ & $1.9^{+5.9\%}_{-3.1\%}$ & $1.6^{+7.3\%}_{-3.8\%}$ \\
%         & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times \%$ & $1.2^{+2.8\%}_{-2.7\%}$ & $0.8^{+4.4\%}_{-4.3\%}$ \\ \hline    
 
%         %TTTT multiply by 10^3
%         % \multirow{3}{*}{$t\bar{t}t\bar{t}$ @ 13~TeV}  & $\sigma_{SM,LO}\times 10^{3}$ & \multicolumn{2}{c}{$4.291^{+63.0\%}_{-36.5\%}$} \\ \cline{3-4}
%         % & $\sigma_{i,LO}^{(1)}\times 10^{3}$ & $0.121^{+50.1\%}_{-31.6\%}$ & $0.068^{+50.7\%}_{-32.5\%}$ \\
%         % & $\sigma_{i,LO}^{(2)}\times 10^{3}$ & $0.094^{+51.0\%}_{-31.9\%}$ & $0.045^{+51.2\%}_{-33.1\%}$ \\
%         % & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times \%$ & $2.81^{+113.1\%}_{-68.1\%}$ & $1.58^{+113.8\%}_{-69.0\%}$ \\
%         % & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times \%$ & $2.18^{+114.1\%}_{-68.4\%}$ & $1.06^{+114.3\%}_{-69.7\%}$ \\ \hline\hline

%         %FL
%         %\multirow{3}{*}{W-hel. FL}  & $F_{SM,LO}$ & \multicolumn{2}{c}{0.296} \\ \cline{3-4}
%         %& $F_{i,LO}^{(1)}\times 10^{3}$ & -0.472 & 0.196 \\
%         %& $F_{i,LO}^{(2)}\times 10^{3}$ & 0.382 & -0.056 \\ \hline
        
%         %F0
%         %\multirow{3}{*}{W-hel. F0}  & $F_{SM,LO}$ & \multicolumn{2}{c}{0.704} \\ \cline{3-4}
%         %& $F_{i,LO}^{(1)}\times 10^{3}$ & 0.471 & -0.197 \\
%         %& $F_{i,LO}^{(2)}\times 10^{3}$ & -0.382 & 0.056 \\ \hline
%     \end{tabular}
%     \caption{Parameterisations for the processes where the considered 4-fermion operators are relevant.}
%     \label{tab:extra_4fermion}
% \end{table}

% \begin{table}[!htpb]
%     \centering
%     \scriptsize
%     \renewcommand\arraystretch{1.5}
%     \begin{tabular}{c|c|c|c}
%         \hline
%         Process & Param. [pb] & $\mathcal{O}_{ut}^8$ & $\mathcal{O}_{dt}^8$ \\ \hline
        
%         %TT TEVATRON
%         \multirow{3}{*}{$t\bar{t}$ @ 1.96~TeV}  & $\sigma_{SM,LO}$ & \multicolumn{2}{c}{$4.95$} \\ \cline{3-4}
%         & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times\%$ & $6.2$ & $1.0$ \\
%         & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times\%$ & $0.5$ & $0.1$ \\ \hline
                
%         % TT 8TEV
%         \multirow{3}{*}{$t\bar{t}$ @ 8~TeV}  & $\sigma_{SM,LO}$ & \multicolumn{2}{c}{$138$} \\ \cline{3-4}
%         & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times\%$ & $1.3$ & $0.8$ \\
%         & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times\%$ & $0.2$ & $0.1$ \\ \hline
                
%         % TT 13TEV
%         \multirow{3}{*}{$t\bar{t}$ @ 13~TeV}  & $\sigma_{SM,LO}$ & \multicolumn{2}{c}{$453$} \\ \cline{3-4}
%         & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times \%$ & $0.9$ & $0.6$ \\
%         & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times \%$ & $0.2$ & $0.1$ \\ \hline
        
%         %TTH
%         \multirow{3}{*}{$t\bar{t}H$ @ 13~TeV}  & $\sigma_{SM,LO}$ & \multicolumn{2}{c}{$0.36$} \\ \cline{3-4}
%         & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times \%$ & $5.7$ & $3.5$ \\
%         & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times \%$ & $2.5$ & $1.3$ \\ \hline    
       
%         %TTY
%         \multirow{3}{*}{$t\bar{t}\gamma$ @ 13~TeV}  & $\sigma_{SM,LO}$ & \multicolumn{2}{c}{$1.32$} \\ \cline{3-4}
%         & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times \%$ & $2.7$ & $1.6$ \\
%         & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times \%$ & $1.1$ & $0.8$ \\ \hline    
        
%         %TTZ
%         \multirow{3}{*}{$t\bar{t}Z$ @ 13~TeV}  & $\sigma_{SM,LO}$ & \multicolumn{2}{c}{$0.51$} \\ \cline{3-4}
%         & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times \%$ & $1.9$ & $1.6$ \\
%         & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times \%$ & $1.2$ & $0.8$ \\ \hline    
 
%         %TTTT multiply by 10^3
%         % \multirow{3}{*}{$t\bar{t}t\bar{t}$ @ 13~TeV}  & $\sigma_{SM,LO}\times 10^{3}$ & \multicolumn{2}{c}{$4.291^{+63.0\%}_{-36.5\%}$} \\ \cline{3-4}
%         % & $\sigma_{i,LO}^{(1)}\times 10^{3}$ & $0.121^{+50.1\%}_{-31.6\%}$ & $0.068^{+50.7\%}_{-32.5\%}$ \\
%         % & $\sigma_{i,LO}^{(2)}\times 10^{3}$ & $0.094^{+51.0\%}_{-31.9\%}$ & $0.045^{+51.2\%}_{-33.1\%}$ \\
%         % & $\frac{\sigma_{i,LO}^{(1)}}{\sigma_{SM,LO}}\times \%$ & $2.81^{+113.1\%}_{-68.1\%}$ & $1.58^{+113.8\%}_{-69.0\%}$ \\
%         % & $\frac{\sigma_{i,LO}^{(2)}}{\sigma_{SM,LO}}\times \%$ & $2.18^{+114.1\%}_{-68.4\%}$ & $1.06^{+114.3\%}_{-69.7\%}$ \\ \hline\hline

%         %FL
%         %\multirow{3}{*}{W-hel. FL}  & $F_{SM,LO}$ & \multicolumn{2}{c}{0.296} \\ \cline{3-4}
%         %& $F_{i,LO}^{(1)}\times 10^{3}$ & -0.472 & 0.196 \\
%         %& $F_{i,LO}^{(2)}\times 10^{3}$ & 0.382 & -0.056 \\ \hline
        
%         %F0
%         %\multirow{3}{*}{W-hel. F0}  & $F_{SM,LO}$ & \multicolumn{2}{c}{0.704} \\ \cline{3-4}
%         %& $F_{i,LO}^{(1)}\times 10^{3}$ & 0.471 & -0.197 \\
%         %& $F_{i,LO}^{(2)}\times 10^{3}$ & -0.382 & 0.056 \\ \hline
%     \end{tabular}
%     \caption{Parameterisations for the processes where the considered 4-fermion operators are relevant.}
%     \label{tab:extra_4fermion}
% \end{table}

\newpage
\restoregeometry
